ISLA: A Coordinate-Free, Measure-Weighted Transformer for Boundary-Driven PDEs

Symmetry is a foundational principle of physics: the behavior of a PDE-governed system does not depend on the coordinate frame, unit system, or mesh used to write it down, and neither should a surrogate model. Yet today's leading neural surrogates lack these invariances and fail under simple transformations of the same problem: for models trained on PDEs of cars in one pose (i.e., translation and rotation), rotating the full PDE raises the surface-pressure error from 4% to more than 100%, and re-sampling its boundary raises it to about 30%. We introduce ISLA (Invariant Slice Attention), a slice-attention transformer for steady, boundary-driven PDEs. Because the boundary determines the interior solution, ISLA encodes the posed boundary once into learned slices and evaluates arbitrary interior points independently through a tree-accelerated learned boundary kernel. Inputs are nondimensionalized in scales computed from the boundary, sums over boundary cells are area-weighted quadratures that converge under mesh refinement, and geometry enters only as distances and relative angles to equivariant slice anchors, making the model equivariant to rigid motions and reflections up to optional token subsampling and tree clustering. On AeroZoo, 2,816 3D flows spanning diverse geometries, poses, physical scales, and boundary conditions, ISLA's mean reference-scaled velocity and pressure errors are 1.9 and 2.2 times lower than the best baseline's. On full AirfRANS, ISLA is second only to an explicit boundary-integral network (GLOBE), with errors 1.6 to 2.6 times lower than the better of Transolver's and GeoTransolver's in every field.

==> macros.tex <==
\ifislapreprint
  \makeatletter
  \renewcommand{\ICML@preprint}{\textit{Preprint.}}
  \makeatother
  \hypersetup{
    pdftitle={ISLA: A Coordinate-Free, Measure-Weighted Transformer for Boundary-Driven PDEs},
    pdfauthor={Peter Sharpe},
    pdfsubject={Preprint}
  }
  \long\def\reviewonly#1{}
  \long\def\preprintonly#1{#1}
  \long\def\reviewpreprint#1#2{#2}
\else
  \long\def\reviewonly#1{#1}
  \long\def\preprintonly#1{}
  \long\def\reviewpreprint#1#2{#1}
\fi

\newcommand{\na}{--}

\makeatletter
\newcommand{\isnset}[2]{\expandafter\gdef\csname isn@#1\endcsname{#2}}
\newcommand{\isn}[1]{\ifcsname isn@#1\endcsname\csname isn@#1\endcsname\else
  \PackageError{islanumbers}{Unknown number key #1}{See generated/numbers.tex}\fi}
\newcommand{\tabinput}[1]{\@@input #1 }
\makeatother

\newcommand{\isla}{ISLA}
\newcommand{\globe}{GLOBE}
\newcommand{\aerozoo}{AeroZoo}
\newcommand{\splitname}[1]{\texttt{\detokenize{#1}}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vr}{\mathbf{r}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vg}{\mathbf{g}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vrbar}{\bar{\mathbf{r}}}
\newcommand{\vm}{\mathbf{m}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vd}{\mathbf{d}}
\newcommand{\gpuname}{NVIDIA GB300 or GB200 GPUs}
\newcommand{\vh}{\mathbf{h}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vZ}{\mathbf{Z}}
\newcommand{\vxi}{\boldsymbol{\xi}}
\newcommand{\vrho}{\boldsymbol{\rho}}
\newcommand{\viota}{\boldsymbol{\iota}}
\newcommand{\vnu}{\boldsymbol{\nu}}
\newcommand{\vphi}{\boldsymbol{\phi}}
\newcommand{\hn}{\hat{\mathbf{n}}}
\newcommand{\hg}{\hat{\mathbf{g}}}
\newcommand{\hu}{\hat{\mathbf{u}}}
\newcommand{\hrho}{\hat{\boldsymbol{\rho}}}
\newcommand{\hnu}{\hat{\boldsymbol{\nu}}}
\newcommand{\htilde}{\tilde{\mathbf{h}}}
\newcommand{\LN}{\operatorname{LN}}
\newcommand{\MLP}{\operatorname{MLP}}
\newcommand{\Rey}{\mathit{Re}}
\newcommand{\cs}{\operatorname{cs}}
\newcommand{\Od}{\mathrm{O}(d)}
\newcommand{\Ed}{\mathrm{E}(d)}
\newcommand{\dd}{\,\mathrm{d}}
\newcommand{\sol}{\mathcal{S}}
\newcommand{\prob}{\mathcal{P}}
\newcommand{\bdry}{\Gamma}
\newcommand{\dom}{\Omega}
\DeclareMathOperator*{\wsoftmax}{softmax}
\DeclareMathOperator{\asinh}{asinh}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\spn}{span}

\definecolor{islablue}{HTML}{1F6FEB}
\definecolor{gtred}{HTML}{D1495B}
\definecolor{tramber}{HTML}{E68A2E}
\definecolor{globegreen}{HTML}{1B998B}

\hyphenation{Driv-Aer-ML Wind-sor-ML Ah-med-ML Airf-RANS Geo-Tran-sol-ver Tran-sol-ver}

